Learning Valuation Distributions from Partial Observation

Auction theory traditionally assumes that bidders' valuation distributions are known to the auctioneer, such as in the celebrated, revenue-optimal Myerson auction. However, this theory does not describe how the auctioneer comes to possess this information. Recently, Cole and Roughgarden [2014] showed that an approximation based on a finite sample of independent draws from each bidder's distribution is sufficient to produce a near-optimal auction. In this work, we consider the problem of learning bidders' valuation distributions from much weaker forms of observations. Specifically, we consider a setting where there is a repeated, sealed-bid auction with $n$ bidders, but all we observe for each round is who won, but not how much they bid or paid. We can also participate (i.e., submit a bid) ourselves, and observe when we win. From this information, our goal is to (approximately) recover the inherently recoverable part of the underlying bid distributions. We also consider extensions where different subsets of bidders participate in each round, and where bidders' valuations have a common-value component added to their independent private values.

==> rw.tex <==
\section{Related Work}\label{sec:rw}

\subsection{Empirical distribution function convergence}
\subsection{Mechanism design through sampling}



\citet{chawla2014data} study a model where the goal is to design
approximately optimal position auctions, when bidders draw their
values i.i.d. from some distribution and bidders then bid according to
some Bayes Nash equilibrium of a (first-price or all-pay)
auction. They show one can invert the best-response function to infer
the valuation distribution from the estimated bid distribution, which
is sufficient to approximately optimize revenue. For their setting,
the length-$n$ bid vectors may be necessary: in order to optimize for
revenue in a position auction, one needs more detailed information
about the lower portions of the distribution.

\citet{cole2014sample} \jmcomment{fill in}

Broadly speaking, our work differs from previous work in this space in
that it assumes very limited observational information. Rather than
assuming all $n$ bids as an observation from a single run of the
auction,, we see only the highest bidder (and, in some cases, the
winning price or bid). 

\begin{itemize}
\item Bulow-Kemperer results, simple vs optimal mech design, single sample
\item Tim and Richard's paper on apx-rev max
\item Kaplan-Meier
\end{itemize}
